A Unified Funnel Restoration SQP Algorithm

We consider nonlinearly constrained optimization problems and discuss a generic double-loop framework consisting of four algorithmic ingredients that unifies a broad range of nonlinear optimization solvers. This framework has been implemented in the open-source solver Uno, a Swiss Army knife-like C++ optimization framework that unifies many nonlinearly constrained nonconvex optimization solvers. We illustrate the framework with a sequential quadratic programming (SQP) algorithm that maintains an acceptable upper bound on the constraint violation, called a funnel, that is monotonically decreased to control the feasibility of the iterates. Infeasible quadratic subproblems are handled by a feasibility restoration strategy. Globalization is controlled by a line search or a trust-region method. We prove global convergence of the trust-region funnel SQP method, building on known results from filter methods. We implement the algorithm in Uno, and we provide extensive test results for the trust-region line-search funnel SQP on small CUTEst instances.

==> 07-colored-pseudocodes_old.tex <==
\section{Detailed Algorithms}
\todo[inline]{I would drop the colored algorithms. David: I agree.}

\begin{algorithm}[htpb!]
\caption{Funnel Strategy: Inner Trust-Region Iterations}
\label{alg:funnel_v3_restoration_funnel_strategy}
\scriptsize
\SetKwProg{myproc}{Procedure}{}{}
  \myproc{$\mathrm{TrustRegionMethod}(\tau^{(k)}, x^{(k)}, \trial{x}^{(k+1,l)}, d_x^{(k,l)}, \kappa_{\mathrm{h}1}, \kappa_{\mathrm{h}2}, \mathit{phase})$}{
  \begin{globalization_mechanism}
  \Repeat{$(\trial{x}^{(k+1,l)}, \trial{\constraintmultipliers}^{(k+1,l)}, \trial{\boundmultipliers}^{(k+1,l)})$ is acceptable} {
		\begin{constraint_relaxation}
      \If{$\mathit{phase}$ = Optimality} {
         $(d_x^{(k,l)}, d_\constraintmultipliers^{(k,l)}, d_\boundmultipliers^{(k,l)}) \gets$ solve $\highlight[subproblem_color]{QP^{(k)}(\highlight[mechanism_color]{\TRradius^{(l)}})}$ \;
      }
      \If{$\highlight[subproblem_color]{QP^{(k)}(\highlight[mechanism_color]{\TRradius^{(l)}})}$ infeasible or $\mathit{phase}$ = Restoration} {
			$(d_x^{(k,l)}, d_\constraintmultipliers^{(k,l)}, d_\boundmultipliers^{(k,l)}) \gets$ solve $\highlight[subproblem_color]{FQP^{(k)}(\highlight[mechanism_color]{\TRradius^{(l)}})}$ starting from $d_x^{(k,l)}$ \;
		}
		\end{constraint_relaxation}
		
		Assemble trial iterate $\trial{x}^{(k+1,l)} \equaldef x^{(k)} + d_x^{(k,l)}$ \;
      Reset the multipliers corresponding to the active trust region \;
      $\mathit{acceptable} \gets \mathit{false}$ \;
      
      \begin{constraint_relaxation}
\eIf{$\|d_x^{(k,l)}\|=0$} {
			$\mathit{acceptable} \gets \mathit{true}$ \;
}{
         
 % possibly switch phases
	\uIf{$\mathit{phase}$ = Optimality and $\highlight[subproblem_color]{QP^{(k)}(\highlight[mechanism_color]{\TRradius^{(l)}})}$ infeasible} {
        $\mathit{phase} \gets$ Restoration \;
	}
	\ElseIf{$\mathit{phase}$ = Restoration and $\highlight[subproblem_color]{QP^{(k)}(\highlight[mechanism_color]{\TRradius^{(l)}})}$ feasible} {
		$\mathit{phase} \gets$ Optimality \;
	}

    \begin{globalization_strategy}
			\uIf{$\mathit{phase}$ = Optimality} {
                \If{Funnel condition $h(\trial{x}^{(k+1,l)}) \leq \kappa \tau^{(k)}$ is satisfied}{
                    \eIf{Switching condition $\Delta m_f^{(k)}(d_x^{(k,l)}) \ge \delta \highlight[constraint_relaxation_color]{(h^{(k)})}^2$ satisfied}{
                        \If{Armijo condition for optimality: $f(x^{(k)}) - f(\trial{x}^{(k+1,l)}) \geq \sigma \Delta m_f^{(k)}(d_x^{(k,l)})$} {
                            $\mathit{acceptable} \gets \mathit{true}$ \;
                        }
                    $\tau^{(k+1)}\gets \tau^{(k)}$\;
                    % LOL\;
                    }{  
                        $\mathit{acceptable} \gets \mathit{true}$\;
                        Reduce funnel: $\tau^{(k+1)} \gets \max \left[\kappa_{\mathrm{h} 1} \tau^{(k)},\, (1-\kappa_{\mathrm{h} 2})h\left(\trial{x}^{(k+1, l)}\right) +\kappa_{\mathrm{h} 2}\tau^{(k)}\right]$\;
                    }
                }
			} 
			\ElseIf {$\mathit{phase}$ = Restoration}{
			    \If{Armijo condition for infeasibility: $h^{(k)} - h(\trial{x}^{(k+1,l)}) \geq \sigma \Delta m_h^{(k)}(d_x^{(k,l)})$} {
	                $\mathit{acceptable} \gets \mathit{true}$ \;
                    Reduce funnel: $\tau^{(k+1)}\gets\max \left[\kappa_{\mathrm{h} 1} \tau^{(k)}, (1-\kappa_{\mathrm{h} 2})h\left(\trial{x}^{(k+1, l)}\right) +\kappa_{\mathrm{h} 2}h^{(k)}\right]$\;
                }
			}
     \end{globalization_strategy}
}
\end{constraint_relaxation}
		
      \eIf{$acceptable$} {
			\If{trust region is active at $d_x^{(k,l)}$} {
				Increase radius $\TRradius^{(l)}$ \;
			}
		}{
			Decrease radius $\TRradius^{(l)}$ \;
		}
		$l \gets l+1$ \;
	}
\end{globalization_mechanism}
}
%}
\end{algorithm}

\begin{algorithm}[htpb!]
\caption{Uno: trust-region funnel restoration SQP.}
\label{alg:framework_tr_funnel_sqp_v3}
\scriptsize
\SetAlgoVlined
\KwIn{$\{\kappa_{\mathrm{h} 1}$, $\kappa_{\mathrm{h} 2}\} \in (0,1)$, $\kappa_{\mathrm{ha}} > 0$, $\kappa_{\mathrm{hr}} > 1$, initial primal-dual iterate $(x^{(0)},\constraintmultipliers^{(0)}, \boundmultipliers^{(0)})$, $\highlight[strategy_color]{\tau^{(0)} = \max \left[\kappa_{\mathrm{ha}},\kappa_{\mathrm{hr}} h^{(0)}\right]}$}
%\KwOut{stationary point}
$k \gets 0$ \;
\begin{constraint_relaxation}
$\mathit{phase} \gets$ Optimality \;
%Initialize $\mathcal{F}_O$ and $\mathcal{F}_R$ \;
\end{constraint_relaxation}

\Repeat{termination criteria are satisfied} {
	\begin{globalization_mechanism}
	Set inner iteration counter $l \gets 0$ \;
	Reset trust-region radius $\TRradius^{(l)} \in [\underline{\TRradius}, \overline{\TRradius}]$ \;
    
    \begin{globalization_strategy}
    \;
    $(\trial{x}^{(k+1,l)}, \trial{\constraintmultipliers}^{(k+1,l)}), \trial{\boundmultipliers}^{(k+1,l)})\gets\mathrm{TrustRegionMethod}(\tau^{(k)}, x^{(k)}, \trial{x}^{(k+1,l)}, d_x^{(k,l)}, \kappa_{\mathrm{h}1}, \kappa_{\mathrm{h}2}, \mathit{phase})$\;
    \end{globalization_strategy}

    
	Update $(x^{(k+1)}, \constraintmultipliers^{(k+1)}, \boundmultipliers^{(k+1)}) \gets (\trial{x}^{(k+1,l)}, \trial{\constraintmultipliers}^{(k+1,l)}), \trial{\boundmultipliers}^{(k+1,l)})$ \;
	\end{globalization_mechanism}
	$k \gets k+1$ \;
}
\Return $(x^{(k)}, \constraintmultipliers^{(k)}, \boundmultipliers^{(k)})$
\end{algorithm}

==> backup-colored-pseudocodes.tex <==
\begin{algorithm}[h!]
\caption{Uno: funnel restoration SQP method.}
\label{alg:funnel_restoration_sqp}
\scriptsize
\SetAlgoVlined
\KwIn{initial primal-dual iterate $(x^{(0)},\constraintmultipliers^{(0)}, \boundmultipliers^{(0)})$}
$k \gets 0$ \;
$\mathit{termination} \gets \mathit{false}$ \;
\begin{constraint_relaxation}
$\mathit{phase} \gets$ Optimality \;
\end{constraint_relaxation}
\begin{globalization_strategy}
$\tau^{(0)} = \max \left[\bar{\tau},\bar{\kappa} h^{(0)}\right]$
\end{globalization_strategy}
\Repeat{$\mathit{termination}$} {
    \begin{globalization_mechanism}
	Compute new acceptable iterate $(x^{(k+1)}, \constraintmultipliers^{(k+1)}, \boundmultipliers^{(k+1})$ (Algorithm \eqref{alg:uno-tr} or \eqref{alg:uno-ls}) \;
    \end{globalization_mechanism}
    \lIf{termination criteria satisfied at $(x^{(k+1)}, \constraintmultipliers^{(k+1)}, \boundmultipliers^{(k+1})$}{$\mathit{termination \gets true}$}
	$k \gets k+1$ \;
}
\Return $(x^{(k)}, \constraintmultipliers^{(k)}, \boundmultipliers^{(k)})$
\end{algorithm}

\begin{algorithm}[h!]
\caption{Uno: trust-region method.}
\label{alg:uno-tr}
\scriptsize
\KwIn{current iterate $(x^{(k)}, \constraintmultipliers^{(k)}, \boundmultipliers^{(k)})$}
\begin{globalization_mechanism}
Set inner iteration counter $l \gets 0$ \;
\Repeat{$(\trial{x}^{(k+1, l)}, \trial{\constraintmultipliers}^{(k+1, l)}, \trial{\boundmultipliers}^{(k+1, l)})$ is acceptable} {
    \begin{constraint_relaxation}
    Compute primal-dual solution $(d^{(k,l)}, \trial{\constraintmultipliers}^{(k+1)}, \trial{\boundmultipliers}^{(k+1)})$ (Algorithm~\ref{alg:direction_computation}) \;
    \end{constraint_relaxation}
    Assemble trial iterate $\trial{x}^{(k+1,l)} \equaldef x^{(k)} + d^{(k, l)}$ \;
    Reset the multipliers corresponding to the active trust region \;
    \begin{constraint_relaxation}
    Determine whether trial iterate is $\mathit{acceptable}$ (Algorithm~\ref{alg:acceptance}) \;
    \end{constraint_relaxation}
    \eIf{$acceptable$} {
        \lIf{trust region is active at $d^{(k,l)}$} {
            increase radius $\TRradius^{(l)}$
        }
    }{
        Decrease radius $\TRradius^{(l)}$ \;
        $l \gets l+1$ \;
    }
}
\end{globalization_mechanism}
\Return $(\trial{x}^{(k+1, l)}, \trial{\constraintmultipliers}^{(k+1, l)}, \trial{\boundmultipliers}^{(k+1, l)})$
\end{algorithm}

\begin{algorithm}[h!]
\caption{Uno: backtracking line search.}
\label{alg:uno-ls}
\scriptsize
\SetAlgoVlined
\KwIn{current iterate $(x^{(k)}, \constraintmultipliers^{(k)}, \boundmultipliers^{(k)})$}
\begin{globalization_mechanism}
\begin{constraint_relaxation}
Compute primal-dual solution $(d^{(k)}, \trial{\constraintmultipliers}^{(k+1)}, \trial{\boundmultipliers}^{(k+1)})$ (Algorithm~\ref{alg:direction_computation}) \;
\end{constraint_relaxation}
$\alpha^{(0)} \gets 1$ \;
Set inner iteration counter $l \gets 0$ \;

\Repeat{$(\trial{x}^{(k+1, l)}, \trial{\constraintmultipliers}^{(k+1, l)}, \trial{\boundmultipliers}^{(k+1, l)})$ is acceptable} {
    Assemble trial iterate $\trial{x}^{(k+1,l)} \equaldef x^{(k)} + \alpha^{(l)} d^{(k)}$ \;
    \begin{constraint_relaxation}
    Determine whether trial iterate is $\mathit{acceptable}$ (Algorithm~\ref{alg:acceptance}) \;
    \end{constraint_relaxation}
    \If{not $acceptable$} {
        Decrease step length $\alpha^{(l)}$ \;
        $l \gets l+1$ \;
    }
    \If{$\alpha^{(l)}$ too small} {
        \begin{constraint_relaxation}
        $\mathit{phase} \gets$ Restoration \;
        $x^\mathit{resto} \gets x^{(k)}$ \;
        Compute primal-dual solution $(d^{(k)}, \trial{\constraintmultipliers}^{(k+1)}, \trial{\boundmultipliers}^{(k+1)})$ (Algorithm~\ref{alg:direction_computation}) \;
        \end{constraint_relaxation}
        $\alpha^{(l)} \gets 1$ \;
    }
}
\end{globalization_mechanism}
\Return $(\trial{x}^{(k+1, l)}, \trial{\constraintmultipliers}^{(k+1, l)}, \trial{\boundmultipliers}^{(k+1, l)})$
\end{algorithm}

\begin{algorithm}[h!]
\caption{Uno: QP direction computation}
\label{alg:direction_computation}
\scriptsize
\SetAlgoVlined
\KwIn{current iterate $(x^{(k)}, \constraintmultipliers^{(k)}, \boundmultipliers^{(k)})$}
\begin{constraint_relaxation}
\If{$\mathit{phase}$ = Optimality} {
    $(d^{(k,l)}, \trial{\constraintmultipliers}^{(k+1)}, \trial{\boundmultipliers}^{(k+1)}) \gets$ solve \colorbox{subproblem_color}{subproblem \ref{eq:QP-subproblem} or \ref{eq:TR-QP}} \;
    
    % switch to feasibility restoration
    \If{\colorbox{subproblem_color}{subproblem} infeasible} {
        $\mathit{phase} \gets$ Restoration \;
        $x^\mathit{resto} \gets x^{(k)}$ \;
        $\constraintmultipliers^{(k)} \gets 0$ \;
    }
}
\If{$\mathit{phase}$ = Restoration} {
    $(d^{(k,l)}, \trial{\constraintmultipliers}^{(k+1)}, \trial{\boundmultipliers}^{(k+1)}) \gets$ solve \colorbox{subproblem_color}{\ref{eq:FQP}} starting from $d^{(k,l)}$ \;
}
\end{constraint_relaxation}
\Return $(d^{(k,l)}, \trial{\constraintmultipliers}^{(k+1)}, \trial{\boundmultipliers}^{(k+1)})$
\end{algorithm}

\begin{algorithm}[h!]
\caption{Uno: funnel acceptance test}
\label{alg:acceptance}
\scriptsize
\KwIn{trial iterate $\trial{x}^{(k+1)}$, direction $d^{(k,l)}$}
\begin{constraint_relaxation}
$\mathit{acceptable} \gets \mathit{false}$ \;
\eIf{$\| d^{(k,l)} \| = 0$} {
    $\mathit{acceptable} \gets \mathit{true}$ \;
}{
    % possibly switch to optimality
    \If{$\mathit{phase}$ = Restoration and \colorbox{subproblem_color}{subproblem} feasible and $\highlight[strategy_color]{h(\trial{x}^{(k+1, l)}) \le \beta \min(\tau^{(k)}, h(x^\mathit{resto}))}$} {
        $\mathit{phase} \gets$ Optimality \;
        \begin{globalization_strategy}
        $\tau^{(k+1)} \gets (1 - \kappa) h(\trial{x}^{(k+1)}) + \kappa \tau^{(k)}$ \;
        \end{globalization_strategy}
    }

    \uIf{$\mathit{phase}$ = Optimality} {
        \begin{globalization_strategy}
        \If{trial iterate is acceptable to funnel: $h(\trial{x}^{(k+1)}) \leq \tau^{(k)}$}{
            \uIf(\tcp*[f]{f-type step}){switching condition is satisfied: $\Delta m_f^{(k)}(d) \ge \delta \left(h^{(k)}\right)^2$}{
                \If{Armijo condition is satisfied: $f^{(k)} - f(\trial{x}^{(k+1)}) \geq \sigma \Delta m_f^{(k)}(d)$} {
                $\mathit{acceptable} \gets \mathit{true}$ \;}
            }
            \ElseIf(\tcp*[f]{h-type step}){funnel is sufficiently reduced: $h(\trial{x}^{(k+1)}) \leq \beta \tau^{(k)}$}{
                $\mathit{acceptable} \gets \mathit{true}$ \;
                $\tau^{(k+1)} \gets (1 - \kappa) h(\trial{x}^{(k+1)}) + \kappa \tau^{(k)}$\;
            }
        }
        \end{globalization_strategy}
    }
    \ElseIf {$\mathit{phase}$ = Restoration}{
        \begin{globalization_strategy}
        \If{Armijo condition is satisfied: $h^{(k)} - h(\trial{x}^{(k+1)}) \ge \sigma \Delta m_h^{(k)}(d)$}{
            $\mathit{acceptable} \gets \mathit{true}$ \;
            % \If{$h(\trial{x}^{(k+1)}) \le \beta \tau^{(k)}$ and $h(\trial{x}^{(k+1)}) \le \beta h(x^\mathit{resto})$}{
            % $\mathit{phase} \gets \mathit{optimality}$ \;
            % $\tau^{(k+1)} \gets (1 - \kappa) h(\trial{x}^{(k+1)}) + \kappa \tau^{(k)}$ \;
            % }
        }
        \end{globalization_strategy}
    }
}
\end{constraint_relaxation}
\Return $\mathit{acceptable}$ \;
\end{algorithm}
